A Tutorial on Complementarity-Based Contact Models for Robotics

Simulating rigid-body dynamics with contact is fundamental to robotics, from motion synthesis and control to mechanism design. Many widely used simulators rely on cone complementarity formulations, whose physical assumptions and numerical solution require substantial background. While excellent surveys, monographs, and course notes exist, they mostly address computational mechanics or computer graphics or document a single simulator. To the best of our knowledge, a self-contained pedagogical treatment for robotics, bringing these formulations and their solvers together with complete derivations and a unified notation, does not yet exist. This tutorial addresses this gap by connecting rigid-body dynamics, conic optimization, and frictional contact. In particular, we explain how complementarity conditions encode non-penetration and frictional dissipation, determining separation, sticking, and sliding without prescribed contact modes. We distinguish equivalent transcriptions from convex relaxations, showing how the latter can introduce artifacts such as lift-off and creep. We examine the existence and uniqueness of motion and contact forces, including the solver's role in selecting among multiple solutions. We then compare first-order and Newton-based methods, explain regularization and proximal strategies, and discuss trade-offs between computational cost, robustness, and physical fidelity. Connections to widely used simulators, optimal control, and differentiable simulation help readers interpret simulation results, choose suitable formulations and solvers, and develop their own contact dynamics routines.

==> contact_notation.tex <==
\RequirePackage{mathtools,amssymb,bm}

\newcommand{\vct}[1]{\bm{#1}}
\newcommand{\gvec}[1]{\mathbf{#1}}
\newcommand{\mat}[1]{\mathbf{#1}}
\newcommand{\cset}[1]{\mathcal{#1}}
\newcommand{\reals}{\mathbb{R}}
\providecommand{\trsp}{\mathsf{T}} %

\newcommand{\vx}{\vct{x}}
\newcommand{\vy}{\vct{y}}
\newcommand{\vz}{\vct{z}}
\newcommand{\vs}{\vct{s}}
\newcommand{\vw}{\vct{w}}
\newcommand{\vp}{\vct{p}}
\newcommand{\vn}{\vct{n}}
\newcommand{\vt}{\vct{t}}
\newcommand{\vg}{\vct{g}}
\newcommand{\va}{\vct{a}}
\newcommand{\vb}{\vct{b}}
\newcommand{\vd}{\vct{d}}
\newcommand{\ve}{\vct{e}}
\newcommand{\vf}{\vct{f}}
\newcommand{\vh}{\vct{h}}
\newcommand{\vu}{\vct{u}}
\renewcommand{\vv}{\vct{v}}
\newcommand{\vlambda}{\vct{\lambda}}
\newcommand{\vmu}{\vct{\mu}}
\newcommand{\vsigma}{\vct{\sigma}}
\newcommand{\vtau}{\vct{\tau}}
\newcommand{\vgamma}{\vct{\gamma}}
\newcommand{\zerovec}{\vct{0}}
\newcommand{\onesvec}{\vct{1}}
\newcommand{\identity}{\mat{I}}
\newcommand{\mA}{\mat{A}}

\newcommand{\gpos}{\gvec{q}}
\newcommand{\gvel}{\gvec{v}}
\newcommand{\gacc}{\gvec{a}}
\newcommand{\gbias}{\gvec{b}}
\newcommand{\forces}{\gvec{f}}
\newcommand{\dualrhs}{\gvec{r}}
\renewcommand{\freeacc}{\gacc_f}
\newcommand{\freevel}{\gvel_f}
\newcommand{\contactvels}{\bar{\vv}}
\newcommand{\freecontactvels}{\contactvels_f}
\newcommand{\contactjac}{\bar{\jacmat}}
\newcommand{\refacc}[1]{\va_{\mathrm{ref},#1}}
\newcommand{\refaccs}{\bar{\va}_{\mathrm{ref}}}
\newcommand{\stacked}[1]{\bar{#1}}
\newcommand{\massmat}{\mat{M}}
\newcommand{\bodymassmat}{\mat{M}}
\newcommand{\coriolismat}{\mat{C}}
\newcommand{\delassus}{\mat{G}}
\newcommand{\regularizer}{\mat{R}}
\newcommand{\regentry}{R} %
\newcommand{\rotmat}{\mat{R}}
\newcommand{\inertiatensor}{\mat{I}}
\newcommand{\kinmap}{\mat{N}}
\newcommand{\frictionbasis}{\mat{B}}
\newcommand{\correction}{\vct{\Gamma}}
\newcommand{\timestep}{\Delta t}
\newcommand{\timehorizon}{T}
\newcommand{\frictioncoef}{\mu}
\newcommand{\stabilization}{\gamma}
\newcommand{\signedgap}{d}
\newcommand{\nq}{n_q}
\newcommand{\nv}{n_v}
\newcommand{\ncontacts}{N}
\newcommand{\nfrictiondirs}{K}

\newcommand{\SOthree}{\ensuremath{\mathrm{SO}(3)}}
\newcommand{\SEthree}{\ensuremath{\mathrm{SE}(3)}}
\newcommand{\sothree}{\ensuremath{\mathfrak{so}(3)}}
\newcommand{\sethree}{\ensuremath{\mathfrak{se}(3)}}
\newcommand{\unitsphere}{\mathbb{S}^{2}}
\newcommand{\ddt}{\frac{\mathrm{d}}{\mathrm{d}t}}
\newcommand{\crossmat}[1]{\left[#1\right]}

\newcommand{\convset}{\cset{C}}
\newcommand{\complset}{\cset{S}} %
\newcommand{\cone}{\cset{K}}
\newcommand{\frictioncone}[1]{\cone_{#1}}
\newcommand{\dualcone}[1]{{#1}^{*}}
\newcommand{\polarcone}[1]{{#1}^{\circ}}

\newcommand{\projop}{\operatorname{P}}
\newcommand{\proj}[1]{\projop_{#1}}
\newcommand{\normalcone}[1]{\operatorname{N}_{#1}}
\newcommand{\normalbasis}[1]{\mat{N}_{#1}}
\newcommand{\jacmat}{\mat{J}}
\newcommand{\jac}[1]{\jacmat_{#1}}
\newcommand{\projjac}[1]{\jac{\proj{#1}}}
\DeclareMathOperator{\linspan}{span}
\DeclareMathOperator{\colspace}{colspace}
\DeclareMathOperator{\concat}{concat}
\DeclareMathOperator{\diagop}{diag}
\DeclareMathOperator{\ncpop}{NCP}
\providecommand{\argmin}{\operatorname*{arg\,min}}
\providecommand{\argmax}{\operatorname*{arg\,max}}

\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}
\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
\DeclarePairedDelimiterX{\inner}[2]{\langle}{\rangle}{#1,\,#2}
\DeclarePairedDelimiterX{\setof}[2]{\lbrace}{\rbrace}{%
  #1\,\delimsize\vert\,#2}


